Collision, explosion and collapse of homoclinic classes

Homoclinic classes of generic $C^1$-diffeomorphisms are maximal transitive sets and pairwise disjoint. We here present a model explaining how two different homoclinic classes may intersect, failing to be disjoint. For that we construct a one-parameter family of diffeomorphisms $(g_s)_{s\in [-1,1]}$ with hyperbolic points $P$ and $Q$ having nontrivial homoclinic classes, such that, for $s>0$, the classes of $P$ and $Q$ are disjoint, for $s<0$, they are equal, and, for $s=0$, their intersection is a saddle-node.

==> bonedim.tex <==





\section{Heterodimensional cycles: a model family}
\label{s.heterodimensional}

In this section, we construct a model one-parameter  
family $(f_t)$ of diffeomorphisms unfolding a heterodimensional cycle.
The study of the semi-local dynamics of $f_t$
will be reduced to the analysis of a one-parameter family of 
endomorphisms with infinitely many discontinuities which
describe the dynamics of $f_t$ in the central direction,
see Section~\ref{s.dinamica1dim}.

Consider a diffeomorphism $f$ with a 
heterodimensional cycle having the  following dynamical
configuration. In local coordinates in $\RR^3$, the cycle is
associated to saddle fixed  points
$Q=(0,0,0)$ and
$P=(0,1,0)$ of indices $2$ and $1$, respectively, such that

\medskip
\noindent
{\bf Partially hyperbolic (semi-local) dynamics of the cycle:}
\begin{itemize}
\item
In the set
$[-1,1]\times [-1,2]\times [-1,1]$ the diffeomorphism has the 
form
$$
f(x,y,z)=
(\la^s x, F(y),
\la^u z)
$$
where
$F\colon [-1,2]\to (-1,2)$ is a strictly increasing
 monotone map with exactly two
fixed points, a source at $0$ and a sink at $1$,  
and
$0<\la^s < d_m < d_M  < \la^u$,  where
$0< d_m
<F^\prime(x)<d_M$
for all $x\in [0,1]$.
\item
 There is $\delta>0$ such that
$F$ in linear in $[-\delta,\delta]$ and 
afine in $[1-\delta,1+\delta]$.
We denote by $\beta>1$ and $0<\lambda<1$,
the eigenvalues of $F$ at
$0$ and $1$, respectively.
\end{itemize}
Observe that
$[-1,1]\times \{(0,0)\}\subset W^s(Q)$,
$\{0\}\times [0,1)\times [-1,1]
\subset W^u(Q)$,
$\{(0,0)\}\times   [-1,1]\subset W^u(P)$,
and
$[-1 ,1]\times (0,1]
\times \{0\}
\subset W^s(Q)$.
Thus 
$\ga= \{0\}\times (0,1)\times \{0\}$ is a normally hyperbolic
curve contained in $W^u(Q)\cap W^s(P)$.

\medskip
\noindent
{\bf Existence and unfolding of the cycle:}
\begin{itemize}
\item
{\bf The cycle:}
There exist $k_0\in \NN$ 
 and a small neighborhood  $U$ of 
$(0,1,-1/2)$ 
such that the restriction of $f^{k_0}$
to $U$ is a translation,
$$
f^{k_0}(x,y,z)=
(x-1/2, y-1, z+1/2).
$$
In particular,
$f^{k_0}(0,1,-1/2)=
(-1/2,0,0)$. Thus 
$W^s(Q)$ and $W^u(P)$ meet
throughout the orbit of the heteroclinic point $(-1/2,0,0)$.
Moreover, observing that
$\{(-1/2,0)\}\times [-1,1]\subset W^u(P)$, we have that  
$(-1/2,0,0)$ is a quasi-transverse heteroclinic point.
\item
{\bf The unfolding of the cycle:} 
Consider the one parameter family $(f_t)$
of diffeomorphisms  coinciding 
with $f$ in 
$[-1,1]\times [-1,2]\times [-1,1]$ and 
the restriction of $f_t^{k_0}$ to $U$ is of the
form
$$
f^{k_0}_t(x,y,z)=
(x-1/2, y-1+t, z+1/2)
=
f^{k_0}(x,y,z)+(0,t,0).
$$
Therefore, for small $t>0$,
$\{(-1/2,t)\}\times [-1,1]\subset W^u(P,f_t)$. Thus
$x_t=(-1/2,t,0)$ is a transverse homoclinic point of
$P$ (for $f_t$). Similarly, $y_t=(-1/2, 0,0)$ is a transverse homoclinic
point of $Q$ (for $f_t$).
\end{itemize}

Consider a small {\em neighborhood of the heterodimensional cycle
associated with $f_0$,\/} that is, an open set $W$ containing the
connexion curve $\ga=\{0\}\times [0,1]\times \{0\}$
and the $f_0$-orbit of the heteroclinic point
$(-1/2,0,0)$.
For small $t$, let $\La_t$ 
be the {\em maximal $f_t$-invariant set in $W$,\/}
$\La_t = \cap_{n\in\ZZ}f_t^{n}(W)$.
We also consider the forward and backward invariant sets in $W$, 
$\La_t^+ = \cap_{n\ge 0}f_t^{-n}(W)$ and
$\La_t^- = \cap_{n\ge 0}f_t^{n}(W)$. 

Suppose that that the eigenvalues $\lambda$ and $\beta$ and
the map $F$  verify the following conditions:
\begin{description}
\item{{\bf (T1)}} 
$\displaystyle{
F^\prime(x) \geq 
\frac{1}{2} \, \frac{1 - \lambda}
{1 - {\beta}^{-1}}}, 
\mbox{ for all } x \in D^+$,
\item{{\bf (T2)}} 
$ (1 - \lambda) < {\beta}^{-1},$ and
\item{{\bf (T3)}} 
$ \displaystyle{ \frac{(1 - \lambda)\,\lambda}{2\,(1 - \beta^{-1})\,\beta}
= \ell  > 1.}$
\end{description}
To have condition (T1) it is enough to consider 
maps $F$ with small distortion in $[0,1]$.
{\em Mather invariant.\/}
(NAO ENTENDI...)
In fact,
to have conditions (T2) and (T3) it is enough to take
$\beta$ close enough to $1$.
%In fact, latter we will consider the case where
%$Q$ is a saddle-node,  see Section~\ref{s.selano}.
Actually, this will be our case, since we will be dealing with the
case where $Q$ is a saddle-node (Section~\ref{s.selano}).
Our first result is:

\begin{theor}
\label{t.lat}
For every  $t>0$ sufficiently small,  
$H(P,f_t)\subset H(Q,f_t)$ and $\La_t\subset H(Q,f_t)$.
\end{theor}

This theorem was stated in \cite{Detds}. Here we give a more conceptual
prove of it, which enables us to introduce some technical
tools to be used systematically later on. 
First, in Section~\ref{s.dinamica1dim} we will introduce the system of iterated
functions associated to the cycle (this approach is motivated by
\cite{DRfund}).
In Section~\ref{s.pontosnaoerrantes}, 
we deduce the theorem
from the results in Section~\ref{s.dinamica1dim}.


\section{One-dimensional dynamics associated to the cycle}
\label{s.dinamica1dim}

Fix $\rho > 0$ small, and consider 
the fundamental domains
of $F$ given by  
$D^+=[\beta^{-1}\rho, \rho]$ and
$D^-=[1-\rho,\lambda(1-\rho)]$
contained in the neighborhoods of $Q$ and $P$
where $F$ is linear.
We can choose $\rho$ such that 
$F^N(D^+)=D^-$ for some
$N\in \NN$ (for notational
simplicity, assume $N=1$).
  The map $F^N = F$
is the {\em transition  from  
$Q$ to $P$.\/}

For each small  $t>0$,  consider the  
{\em scaled fundamental  domains\/} $D_t^\pm$ defined as follows. 
Let
$D^-_t = [1-t,\lambda (1-t)]$ 
and define
$k_t$ as the smaller $k \in \NN$ with
$F^{-k}(D^-_t) \subset [0,t]$. We define
$$
D_t^+ = [a_t,b_t] = 
[\beta^{-1} (b_t),b_t]=
 F^{-k_t}(D^-_t),
\quad
\mbox{where}
\quad
\beta^{-2} t < a_t<b_t\le t.
$$

We next define an expanding  map
$R_t$, 
$R_t\colon D^+_t\to D_t^+$, with discontinuities that will   
describe
 the dynamics 
(in the central 
direction) of the return map of  $f_t$ defined on 
$[-1,1]\times D_t^+ \times [-1,1]$. For each small $t>0$
define the {\em transition map $T_t$ from  $D_t^+$ to $D_t^-$\/} by
$$
T_t \colon  D_t^+ \rightarrow D_t^-,
\quad
x\mapsto T_t(x)=F^{k_t}(x).
$$
\begin{lemm}
\label{l.Tt}
The map 
$T_t$
verifies $T_t^\prime(x)>\ell>1$ for all $x\in D_t^+$, 
where
$\ell$ is as in condition {\bf (T3)}.
\end{lemm}

\begin{demo}
Given $x\in D_t^+$ let 
$k_t=n_t(x)+1+m_t(x)$, where
$F^{n_t(x)}(x)\in D^+$ and 
$F^{i}(x)\not \in D^+$ for all $1 \leq i < n_t(x)$.
We claim that
\begin{equation}
\label{e.blnt} 
\frac {1}{\beta \, t} \leq {\beta}^{n_t(x)} \leq \frac{{\beta}^2}{t}
\quad
\mbox{and}
\quad
\lambda\,  t \le {\lambda}^{m_t(x)} \le \frac{t}{\lambda}.
\end{equation}
For first pair of inequalities just note 
$x\in D_t^+ \subset (\beta^{-2} \, t, t]$ 
and
$\beta^{n_t(x)}\, x \in [\beta^{-1},1]$.
The other ones follow
analogously.

Observing that $T_t(x) = \la^{m_t(x)} \, F (\be^{n_t(x)}\,x)$,
hypothesis (T3) and the estimates in 
(\ref{e.blnt}) give
$$
|T_t^\prime (x)| = \la^{m_t(x)}\, |F^\prime (x)| \, {\be}^{n_t(x)} \geq
(\lambda \, t) \,
\left( \frac{1}{2} \,
\frac{1 - \lambda}{1 - {\beta}^{-1}}\right) \,
\left( \frac{1}{\beta \,t} \right) \, 
= \frac{1}{2} \, \frac{\la\, (1 - \la)}{\beta\, (1 - \beta^{-1})} = \ell > 1,
$$
as we claimed.
\end{demo}

\medskip
Since $T_t(x) \in D_t^-=[1-t,1-\lambda t]$ for all $x \in D_t^+$,
we can define the map $G_t$ by
$$
G_t \colon D_t^+ \rightarrow [0,t],
\quad
x \mapsto G_t(x) = T_t(x) + (t-1).
$$

\begin{rema}
\label{r.Gt}
The map $G_t$ is monotone increasing and
$G_t(D_t^+)=[0,t(1-\lambda)]$.
\end{rema}


\begin{clai}
\label{c.ai>0}
Let $(a_t,b_t] = \tilde{D}_t^+\subset D_t^+$.
Given  $x\in \tilde{D}_t^+$ let $i(x)\in \ZZ$ 
be the minimum $i$ with
${\beta}^i(G_t(x)) \in D^+_t$. 
Then there is $i_0>0$ (maximum with such a property)
such that $i(x)\ge i_0$ for all $x \in\tilde D_t^+$. 
\end{clai}



\begin{demo}
Observe first that, since
$\tilde{D}_t^+ \subset [{\beta}^{-2}t, t]$,  
$b_t\in (\beta^{-1}\, t,t]$.
On the other hand, from Remark~\ref{r.Gt}
and $(1 - \la) < \beta^{-1}$ (condition (T2)), 
$G_t(\tilde{D}^+_t) = (0, t\,(1 - \lambda)]
\subset
(0, \beta^{-1}\, t)$. 
Thus 
the right extreme of 
$G_t(\tilde{D}_t^+)$ is less than  the
left extreme of $D_t^+$, hence $i(x)>0$ for all $x\in \tilde D_t^+$,
ending the proof of the claim.
\end{demo}

Finally,
the return map $R_t$ is defined by
$$
R_t\colon \tilde{D}^+_t \rightarrow D^+_t, 
\quad
R_t(x)={\beta}^{i(x)}(G_t(x))=\beta^{i(x)}\, (T_t(x)+(t-1)).
$$
Next we study the dynamics of $R_t$: the
map $R_t$ 
is uniformly expanding and has
(infinitely many) 
discontinuities 
where the lateral derivatives are well defined. 
These discontinuities will play a key role in our constructions.
   
The definition of 
$i_0\in \NN$ in Claim~\ref{c.ai>0}
implies that
$\beta^{-i_0}(a_t) \in G_t(D_t^+)$.  
For each $i\ge i_0$ define
$d_i\in \tilde{D}_t^+$ by  $G_t(d_{i}) = \beta^{-i}(a_t)$. 
By construction, the sequence $(d_i)_{i\ge i_0}$
verifies the following:
\begin{itemize}
\item
$d_{i+1}< d_i$ and
$d_i\to a_t$, 
\item
Let $[d_{i+1}, d_i]=I_i$, $i > i_0$, and
$I_{i_0} = [d_{i_0},b_t]$.
The map $R_t$ is continuous and 
strictly increasing in the interior of each interval $I_i$.
We continuously extend $R_t$ to the whole $I_i$,
obtaining a bi-valuated return map $R_t$ with
$R_t(d_i)=\{a_t, F(a_t)=b_t\}$ for all $i>i_0$.
In particular, the restriction of $R_t$ to any $I_i$, $i>i_0$, 
is onto.
We let $R_t(b_t)=c_t\le b_t$.
\end{itemize}
The main properties of $R_t$ are summarized in the next lemma.

\begin{lemm}
\label{l.Rtexpansora}
The restriction of $R_t$ to each interval
$I_i, i > i_0$, is onto and 
$R_t^\prime(x)>\ell >1$ for all $x\in (a_t,b_t]$
(if $x=d_i$ this means that the lateral derivatives of
$R_t$ at $x$ are  greater than $\ell$).
Moreover,
$G_t(R_t(d_i)) = 0$
for all $i \geq i_0$.
\end{lemm}
The  expansiveness
of $R_t$ follows 
from Lemma \ref{l.Tt} and Claim~\ref{c.ai>0}. Condition 
$G_t(R_t(d_i))=0$ follows from
$R_t(d_i)=a_t$ and
$G_t(a_t)=0$.

\begin{lemm}
\label{l.descont}
Consider a small $t>0$ 
and   an open subinterval $J$  of $\tilde{D}^+_t$. Then there is  
a first $k \in \NN \cup \{0\}$ 
such that $R_t^k(J)$  contains a discontinuity $d_j$ of $R_t$.
In particular, there is
$x\in J$ 
such that
$G_t(R_t^k(x))=0.$
\end{lemm}

\begin{demo}
If the interval  $J$ contains a discontinuity we are done.
Otherwise, let $i>0$ be such that the intervals $J$, $R_t(J), 
\dots, R_t^i(J)$ do not contain
discontinuities. Thus,
for each $k\in \{0,\dots, i\}$, there is $i_k\ge i_0$ such that
$R_t^k(J)\subset I_{i_k}$.
Lemma~\ref{l.Rtexpansora}
implies that
$|R_t^k(J)|\ge \ell^k |J|$, $\ell>1$,
for all  $k\in \{0,\dots, i\}$.
Since the size of the intervals $I_i$ is upper bounded,
this inequality implies that
there is a first $m\in \NN$
such that
$R_t^m(J)$ 
is not contained in any $I_i$, thus
it intersects the set of  discontinuities.
\end{demo}

\section{The maximal invariant set: Proof of Theorem~\ref{t.lat}}
\label{s.pontosnaoerrantes}


Next proposition is the main technical result of this section. 
Heuristically, it 
 means that the one-dimensional stable 
manifold of $Q$ topologically behaves as a 
two-dimensional manifold.


\begin{prop}
\label{p.chi}
For every 
small $t>0$ and every
two-disk $\chi$ with 
$W^s(P,f_t)\pitchfork \chi\ne \emptyset$
one has
$W^s(Q,f_t)\pitchfork \chi\ne \emptyset$.
In particular, $W^s(P,f_t)$ is contained
in the closure
of $W^s(Q,f_t)$.         
\end{prop}

\paragraph{Proof of Theorem~\ref{t.lat}.}
The inclusion $H(P,f_t)\subset H(Q,f_t)$ in Theorem~\ref{t.lat}
is  deduced from Proposition~\ref{p.chi} as follows. 
By the definition of $H(P,f_t)$, it suffices 
to see that any  
$x\in W^s(P,f_t)\pitchfork W^u(P,f_t)$
is accumulated by homoclinic points of $Q$.
The geometric configuration of the cycle implies that
$W^u(P,f_t)\subset
\mbox{closure\,} (W^u(Q,f_t))$. Thus,
given any $x\in H(P,f_t)$
and any $n>0$, there is a disk
$\Delta_n$ simultaneously contained in $W^u(Q,f_t)$
and in the ball of  radius $1/n$ centered at  
$x$ such that its   
interior transversely meets $W^s(P,f_t)$.
By Proposition~\ref{p.chi},  
$\De_n\pitchfork W^s(Q,f_t)\ne \emptyset$. Thus there is $y_n\in
\De_n\cap H(Q,f_t)$. 
By construction, $y_n\to x$,
 ending the proof of the inclusion
$H(P,f_t)\subset H(Q,f_t)$.


\medskip


\subsection{Homoclinic classes - Proof of Proposition~\ref{p.chi}}
\label{ss.homoclinicclasses}

We now go into the details of the
proof of Proposition~\ref{p.chi}. We
first introduce some definitions.

%\begin{defi}
%\label{d.strips}
%$\,$
\begin{itemize}
\item
A set
$\Delta \subset [-1,1]\times [-1,2]\times [-1,1]$ 
is a {\em vertical strip\/}
if 
$\Delta = \{x_1\}\times[l_1,l_2]\times[r_1,r_2]$,
where $l_1<l_2$ and  $r_1<0<r_2$.
The segment 
$\{x_1\}\times [l_1,l_2]\times \{0\}$ is the {\em basis\/} of $\De$. The
{\em width\/} and the 
{\em height\/} of $\Delta$ are
 $w(\Delta)=(l_2-l_1)$ and 
$h(\Delta)=(r_2-r_1)$. 
The strip $\De$ is {\em complete\/} if
$r_2=1$ and $r_1=-1$, 
{\em well located\/} if
$[l_1,l_2]$ is contained in the interior of $D_t^+$,
and {\em perfect\/}
if it simultaneously is complete and well located.
\item
A subset 
$J\subset  [-1,1]\times [-1,2]\times [-1,1]$ 
is a {\em vertical segment\/} if  
$J = \{x_1\}\times\{l_1\}\times[r_1,r_2]$, where
$r_1<0<r_2$.
The  {\rm height\/} of $J$ is   $h(J)=(r_2-r_1)$. 
As above, the  segment $J$ 
is {\em complete\/} if  
$r_1=-1$ and $r_2=1$, {\em well located\/}
if $l_1$
 is in the interior of
$D_t^+$, and {\em perfect\/} if it simultaneously is complete and well
located.
\item
A vertical segment $J$ 
(resp. strip $\De$) 
is {\em at the right
of $Q$\/} if
$l_1\in (0,1]$. 
\end{itemize}
%\end{defi}

Denote by $\De(\{x\}\times \alpha \times \{0\})$
(resp. $J (x,y,0)$) the {\em unique\/}
complete vertical strip (resp. segment)
with basis $\{x\}\times \alpha\times \{0\}$
(resp $(x,y,0)$).
The following algorithm associates to perfect disks and strips
their successors:

Obs: Lembre que "disk" nao foi definido

\begin{algo}
\label{a.algoritmo}
Let 
$\De=\De(\{x\}\times \alpha \times \{0\})$
a perfect strip. 
Let $\cG_t(\De)$  be
the  perfect strip
such that:
\begin{itemize}
\item
the basis of
$\cG_t(\De)$ 
is of the form $(\{x^\prime\}\times 
G_t(\alpha) \times \{0\})$, where $x^\prime=\la_s^{k_t} \, x-1/2$,
\item
$\cG_t(\De)$ is contained in $f_t^{k_t}(\De)$
(where $F^{k_t}(D_t^+)= D_t^-$).
\end{itemize}
Suppose now that $\alpha$ does not contain discontinuities, i.e.
$\alpha\subset (d_i,d_{i+1})$ for some $i$. 
Define $\cR_t(\De)$  as
the  perfect disk
such that:
\begin{itemize}
\item
the basis of
$\cR_t(\De)$ 
is of the form $(\{x^\prime\}\times 
R_t(\alpha) \times \{0\})$,  where
$x^\prime =\la_s^i(\la_s^{k_t} \, x-1/2)$,
\item
$\cR_t(\De)$ is contained in $f_t^{k_t+i}(\De)$.
\end{itemize}
Similarly, to a perfect segment $J =J (x,y,0)$ 
we associate
 perfect segments $\cG_t(J)$ and $\cR_t(J)$
(provided $y\ne d_i$ for all $i$).
\end{algo}

In fact, the disks $\cG_t(\De)$ and $\cR_t(\De)$ in Algorithm~\ref{a.algoritmo}
are obtained as follows.
Given a set $A$ and a point $x\in A$,  denote by
$C(x,A)$ the connected component of $A$ containing $x$. 
Consider a small tubular neighborhood $V$ of
$f^{k_0}_0(\{0,0\}\times [-1,1])\subset W^u(P,f_0)$,
$k_0$ as in 
the definition of the cycle in Section~\ref{s.heterodimensional},
$$
\cG_t(\De)=
C(f^{k_t}_t(x,y,0), f_t^{k_t}(\De) \cap V)
\cap [-1,1]^3,
\qquad
\cR_t(\De)=
C(f^{i}_t(x^\prime,y^\prime,0), f_t^{k_t+i}(\De) \cap V)
\cap [-1,1]^3),
$$
where
$(x,y,0)$ is any point in the basis of $\De$, 
$x^\prime=(\la_s^{k_t} \, x-1/2)$, and  $y^\prime\in G_t(\alpha)$.
The construction for the successors of the segments is analogous.



\begin{lemm}
\label{l.Wuptsegtovert}
The manifold $W^u(P,f_t)$ contains a perfect 
segment for all small  $t>0$.
\end{lemm}

\begin{demo}
Consider the transverse homoclinic point 
$x_t=(-1/2,t,0)$ of
$P$ (for $f_t$).
Recall that
$t\ge b_t$ and $\beta^{-1} \,t\in D_t^+=[a_t,b_t]$.
Let us assume that 
$t> b_t$,
and thus $\beta^{-1} t\in (a_t,b_t)$
(the case $t=b_t$ follows similarly, so it will be omitted).

Consider the complete vertical segment $\cR_t(J)$, where 
$J=
J(-\la_s^{-1}/2, \be^{-1}t,0)\subset W^u(P,f_t)$.
If $R_t(\be^{-1} t)$ belong to the interior of $D_t^+$,
then $\cR_t(J)\subset W^u(P,f_t)$ is
the announced segment.
Otherwise,
$R_t(\be^{-1} t)=b_t$ and there is
a homoclinic point of
$P$ of the form $(x^\prime, b_t,0)$.
Using the  $\la$-lemma and the 
product structure of the cycle, 
one gets  
homoclinic points  $(x_n, y_n,0)$ of $P$ 
and  complete
segments $J_n=J(x_n, y_n,0)\subset W^u(P,f_t)$
such that 
$x_n\to x^\prime$, $y_n\to b_t$, and 
$y_n$ is increasing.
 Thus $y_n$ belongs to the interior of $D_t^+$ for every
big $n$ and $J_n\subset W^u(P,f_t)$ is perfect.
\end{demo}

For clearness we first prove
Proposition~\ref{p.chi} 
in the following special case:

\begin{prop}
\label{p.chip}
Let $\chi \subset [-1,1]\times [-1,2]\times [-1,1]$ be a set of the form 
$\{x\} \times A$, where $A$ is a disk 
of $\RR^2$ whose interior contains a point of the form $(y,0)$ with
$y\in (0,2)$.
Then $\chi$  intersects transversely $W^s(Q,f_t)$.
\end{prop}

We claim that is enough to prove the 
Proposition~\ref{p.chip} for perfect strips:

\begin{lemm}
\label{l.faixavertical}
Let $\De$ be a perfect
strip. 
Then there is $k \in \NN$
such that
$f_t^{k}(\De) \pitchfork W^s(Q,f_t) \neq \emptyset.$
\end{lemm}

\begin{demo}
Suppose that $\De=\De(\{x_0\}\times \alpha\times \{0\})$, 
$\alpha$ in the interior of $D^+_t$. 
By Lemma~\ref{l.descont}, 
there exist $y_0$ in the interior of $\alpha$ 
and  $k\in \NN$
such that $G_t(R^k_t(x_0))=0$.
Thus the vertical strip
$\cG_t(\cR^k_t(\De))$ (contained in the forward orbit of
$\de$) transversely intersects $[-1,1]\times \{(0,0)\}
\subset W^s(Q,f_t)$.
\end{demo}

\medskip
\noindent
{\bf Proof of 
Proposition~\ref{p.chip}:}
By Lemma~\ref{l.Wuptsegtovert},
$W^u(P,f_t)$
contains a perfect vertical segment $J$.
By definition, $\chi$ meets transversely 
$W^s(P,f_t)$, which implies, by the
$\lambda$-lemma, that the
forward orbit of 
$\chi$ contains a sequence of complete  strips $\chi_n$
accumulating to $J$. 
Thus $\chi_n$
contains a perfect  strip for all  $n$ large. 
Lemma~\ref{l.faixavertical}
now implies that $\chi_n$  (and thus $\chi$) 
transversely meets $W^s(Q,f_t)$, ending the proof of the proposition.
\hfill$\Box$


\medskip
\noindent
{\bf Proof of 
Proposition~\ref{p.chi}:}
We can  assume that
$\chi$ is  transverse to
$W^s_{loc}(P,f_t)$ and contained in 
$[-1,1]\times [-1,2]\times [-1,1]$.
If  $\chi$ contains a 
subset of the form $\{x\}\times A$, where  
$A$ is an open subset of $\RR^2$ containing $(0,0)$,    
Proposition~\ref{p.chip} implies the result.
For the general case, consider
 a point $(x_0,y_0,0)$ in the interior of
$\chi\pitchfork W^s_{loc}(P, f_t)$ and
the  vertical strip  
$$
\Sigma_n=\{x_0\}\times
[y_0-1/n, y_0+1/n]\times
[-1/n,1/n].
$$
This strip 
verifies the hypotheses of 
Proposition~\ref{p.chip},
hence there is $(x_0,y_n,z_n)\in \Sigma_n \pitchfork W^s(Q,f_t)$
such that 
$H_n=
[-1,1]\times \{(y_n,z_n)\}
\subset W^s(Q,f_t)$.
Since 
$(x_0,y_n,z_n)\to (x_0,y_0,0)$,
it is immediate that 
$H_n$ meets transversely  $\chi$ for all large $n$, ending the proof of the
proposition.
\hfill$\Box$

\subsection{The maximal $f_t$-invariant set}
\label{ss.maximalinvariant}

To prove the first part of Theorem~\ref{t.lat} 
($\La_t\subset H(Q,f_t)$)
let
$V_0$ be the connected component of $W$ containing the heteroclinic
point $(-1/2,0,0)$.
There are two types 
of points of $\La_t$: 
(a) those points whose orbit
does not meet $V_0$ (i.e., the set 
$\{0\}\times [0,1]\times \{0\}$) 
and (b) those having an iterate in $V_0$.

We claim that
every point of type (a) belongs to $H(Q,f_t)$: given 
any $(0,x,0)$, $x\in (0,1)$, consider the disk 
$\De_n
=\{0\}\times [x-1/n,x+1/n]\times [-1/n,+1/n]
\subset W^u(Q,f_t)$. By Proposition~\ref{p.chi}, 
$\De_n\pitchfork W(Q,f_t)\ne \emptyset$ and thus
$\De_n \cap H(Q,f_t)\ne \emptyset$. Since this holds for all $n\in \NN$,
$(0,x,0)\in H(Q,f_t)$. 

For points $w\in \La_t$ of type (b),
after replacing $w$ by
some iterate of it,  we can assume that $w\in V_0$.
Consider the sequence
$(n_i(w))_{i \in \cI(w)}$ associated to $w$,  where 
$\cI(w) \subset \ZZ$ is an interval in $\ZZ$,
inductively defined as follows:
let $n_0(w)=0$ and,  assuming defined $n_j(w)$, $j\ge 0$,
we define
$n_{j+1}(w)$ as the first integer $k>n_j(w)$ such that
$f_t^k(w) \in V_0$.
If the forward orbit of $w$ does not return to 
$V_0$ for every $k>n_j(w)$ then $j$ is the right extreme
of $\cI(x)$. 
We argue analogously for negative $j$, assuming defined $n_j(x)$, 
$j\le 0$,
$n_{j-1}(w)$ is the first negative
integer  $k<n_j(w)$ with
$f_t^k(w) \in V_0$. 
If the backward orbit of $w$ does not return to $V_0$ then
$j$ is the left
extreme of $\cI(w)$.

Define $\cI^+_t(\infty)$ and $\cI^+_t(b)$ as the subsets of 
$\La_t\cap V_0$
of points $w$ such that
$\cI(w)$ is not upper bounded and $\cI(w)$ is 
upper bounded, respectively. The subsets
$\cI^-(\infty)$ and $\cI^-(b)$ are defined similarly.
We let 
$\cI^\pm (\infty)=\cI^+(\infty)\cap 
\cI^-(\infty)$ and
$\cI^\pm (b)=\cI^+(b)\cap 
\cI^-(b)$.
We borrow from
\cite[Lemma 4.1]{DRnon} the following lemma whose proof is 
straightforward:

\begin{lemm} 
\label{l.classificacao}
For every small $t>0$,   
$\cI_t^+(b)\subset W^s(P,f_t)\cup W^s(Q,f_t)$ and
$\cI_t^-(b)\subset W^u(P,f_t)\cup W^u(Q,f_t)$. 
\end{lemm}


Next result 
immediately follows by  
observing that 
$f_t$ (resp. $f_t^{-1}$)
exponentially expands the vertical (resp. horizontal) segments:

\begin{rema}
\label{r.expansaonegativa}
Let $w=(x,y,z)\in \cI_t^+(\infty)$ (resp.
$w\in \cI_t^-(\infty)$).
Then 
$\{(x,y)\}\times [z-\ve,z+\ve]
\pitchfork W^s(P,f_t)\ne \emptyset$
(resp. 
 $[x-\ve,x+\ve]\times \{(y,z)\}
\pitchfork W^u(Q,f_t)\ne \emptyset$)
for every $\varepsilon>0$. 
\end{rema}

To prove the theorem we consider the following four cases.  

\medskip

\noindent
{\bf Case (i):
$w=(x,y,z)\in \cI^+_t(\infty)
\cap \cI^-_t(b)$.} 

By Remark~\ref{r.expansaonegativa},
there is a sequence 
$w_n=(x,y,z_n)\in W^s(P,f_t)$ with $w_n\to w$.
We claim that $w_n\in H(Q,f_t)$ for all large $n$.
Thus $w\in H(Q,f_t)$.

Since the distances between the backward iterates of
$w_n$ and $w$ exponentially decrease,
we get that $w_n\in \La_t$. 
Since $w\in \cI^-_t(b)$,
Lemma~\ref{l.classificacao}
implies that
 $w, w_n\in W^u(P,f_t)\cup W^u(Q,f_t)$.
If $w_n\in W^u(P,f_t)$, then $w_n\in H(P,f_t)\subset
H(Q,f_t)$ and we are done.
Otherwise,  
the cycle configuration  gives, 
for each big $k$, a small vertical
strip $\De_k$ of diameter less than $1/k$, 
whose interior is contained in 
$W^u(Q,f_t)$ and whose closure contains $w_n$.
Moreover, since $w_n\in W^s(P,f_t)$,
we can assume that
$\De_k\pitchfork W^s(P,f_t)$.
Thus,
by Proposition~\ref{p.chi}, 
$W^s(Q,f_t)$ transverselly intersects the interior of
$\De_k$.
Hence,
since the interior of  $\De_k$ is contained in $W^u(Q,f_t)$, 
$\De_k$ contains a homoclinic
point $y_k$ of $Q$. From
$\mbox{diam}(\De_k)\to 0$, we get $y_k\to w_n$, which implies
 $w_n\in H(Q,f_t)$. 


\medskip
\noindent
{\bf Case (ii):
$w=(x,y,z)\in \cI_t^\pm(\infty)$.}  

We claim that $w$ is accumulated by points
$w_n\in \cI_t^+(\infty)\cap \cI^-_t(b)$, and 
the result follows from the first case.
To prove the claim observe that,
by Remark~\ref{r.expansaonegativa},
there is a sequence 
$w_n=(x_n,y,z)\in W^u(Q,f_t)$ with $w_n\to w$.
Since the distances between the forward iterates of
$w_n$ and $w$ exponentially decrease,
$w_n\in \La_t$. 
This also implies that
$w_n\in \cI^+_t(\infty)$.
Finally, 
$w_n\in W^u(Q,f_t)$ implies 
$w_n\in \cI^+_t(b)$, ending the proof of the claim.

\medskip
\noindent
{\bf Case (iii):
$w=(x,y,z)\in \cI_t^+(b)\cap \cI^-_t(\infty)$.}  

By Lemma~\ref{l.classificacao},
 $w \in W^s(P,f_t)\cup W^s(Q,f_t)$ and, by replacing $w$ by a forward iterate,
 we can assume that $w=(x,y,0)$, $y\ge 0$. 
Remark~\ref{r.expansaonegativa} gives a sequence 
$w_n=(x_n,y,0)\in W^u(Q,f_t)$ with  $w_n\to w$.
For each $n$, there is a vertical disk $\De_n\subset  W^u(Q,f_t)$ 
centered at  $w_n$, of 
diameter less than  $1/n$. Clearly, $\De_n$ intersects transversely 
$W^s(P,f_t)$. Thus, by
Proposition~\ref{p.chi},   
$\De_n \pitchfork W^s(Q,f_t) \neq \emptyset$. As in the previous cases, this
implies that
$\De_n \cap H(Q,f_t) \neq \emptyset$ for all  $n$ large,
thus $w\in H(P,f_t)$


\medskip
\noindent
{\bf Case (iv):
$w\in \cI^\pm_t(b)$.}

By  Lemma~\ref{l.classificacao},
there are four possibilities:
(1) $w \in W^s(Q,f_t) \cap W^u(Q,f_t)$,
(2) $w \in W^s(P,f_t) \cap W^u(P,f_t)$,
(3) $w \in W^s(P,f_t) \cap W^u(Q,f_t)$,
and (4)
 $w \in W^u(P,f_t) \cap W^s(Q,f_t)$.
Recall that the intersections above are transverse or quasi-transverse, 
depending on the case. Hence, 
in case (1), $w\in H(Q,f_t)$ and, in
case (2), $w\in H(P,f_t)\subset H(Q,f_t)$. 
In case (3),
the  proof of $\{0\}\times [0,1]\times \{0\}\subset H(Q,f_t)$ 
implies that
$w\in H(Q,f_t)$: 
just observe that for every disk $\De\subset W^u(Q,f_t)$ containing $w$,
one has $W^s(P,f_t)\pitchfork \De\ne 
\emptyset$, thus $\Sigma\cap H(Q,f_t)\ne \emptyset$.
It still remains the case
$w \in W^s(Q,f_t) \cap W^u(P,f_t)$.
By replacing $w$ by a forward iterate, we can assume
that $w=(x,0,0)$, $x\in [-1,1]$, and the following lemma easily implies 
case (4):

\begin{lemm}
\label{l.zninfty}
Let $w=(x,0,0) \in V_0 \cap (W^s(Q,f_t) \cap W^u(P,f_t))$.
Then there is a  sequence
$w_n\to w$ with 
$w_n\in \cI_t^+(\infty)$.
\end{lemm}
%The  previous cases imply that 
%$w_n \in H(Q,f_t)$, and thus $w\in H(Q,f_t)$.

\begin{demo}
For each $n\in \NN$,
consider the rectangle
$R_n(x) = \{x\}\times [0, 1/n]\times [-1/n,1/n]$.

\begin{clai}
There exists $z_n$ in  $R_n(x)\in \La_t^+$ 
whose forward  returns to  $V_0$ infinitely many times.
\end{clai}

Assuming this claim, we now finish the proof of the lemma:
imilarly as in Remark~\ref{r.expansaonegativa},
but considering now points in $\La_t^+$, 
we have that the point  $z_n=(x_n,y_n,z_n)$ is 
accumulated by points $z_n^m\in W^u(Q,f_t)$
of the form $(x_n^m, y_n, z_n)$. Since the distances between the forward 
iterates of $z_n$ and $z_n^m$ decrease, the forward orbit of $z_n^m$
is contained in $W$ and returns infinitely many times to $V_0$. 
On the other hand,
since $z_n^m\in W^u(Q,f_t)$, its backward orbits
also is in $W$. Thus the whole orbit of $z_n^m$ is in $W$, so
$z_n^m\in \La_t$ and $z_n^m\in \cI_t^+(\infty)$.
By the cases considered above, $z_n^m\in H(Q,f_t)$, thus
$z_n\in H(Q,f_t)$.


To prove the claim, we exhibit a sequence 
$(R_n^i(x))_{i \in \NN}$
of nested (compact) 
sub-rectangles
of $R_n(x)$ 
such that
the forward orbit of each point of $R_n^{i}(x)$ 
returns to $V_0$ at least 
$i$ times. 
The claim follows 
taking  any point $z_n$ in the non-empty intersection
$\cap_{i \geq 0}R_n^i(x)$.

\begin{fact}
\label{l.retangulo}
Let $R=R_n(x)$, 
$1/n<t$. Then 
there is
$i=i(R) \in \NN$ 
such that, for every 
$j \geq i$,
$f_t^j(R)$ contains a  rectangle
$\Ga(R,j) $ of the form
$\{a\}\times [0,1/n]\times [-1/n,1/n]$. 
 \end{fact}

\begin{demo} 
Define
$N_t$ as the smaller $i \in \NN$ such that
$F^{i}(1/n)\in (1-t+1/n,1)$
and let 
$e=(1-t+1/n+g)=F^{N_t}(1/n)$, $g\in (0,t-1/n)$.
The definition of the unfolding of the cycle implies that,
for each $j\ge 0$,
$f_t^{N_t+j}(R_n(x))$ contains a rectangle of the form
$$
\{\la_s^{N_t+j}(x)-1/2\}
\times 
[0,t+\la^j(g+1/n-t)]
\times [-1,1]
%\subset 
%\{\la_s^{N_t+j}(x)-1/2\}
%\times 
%[0,t+(g+1/n-t)]
%\times [-1,1]\\
\supset
\{\la_s^{N_t+j}(x)-1/2\}
\times 
[0,g+1/n]
\times [-1,1].
$$
This finishes the proof of the fact.
\end{demo}

To prove the Lemma~\ref{l.zninfty},
consider   $R_n(x) = R(0)$ and, using Fact~\ref{l.retangulo}, let 
$R(1)=\Ga (R(0), i(R(0))$.
Write
$R^1 =  f_t^{-i_0}({R}(1)) \subset R(0)$.
Assume inductively defined
numbers $i_{k-1}$ and  
rectangles $R(k)$ and $R^k$ for every $k\in \{0,\dots,j\}$
as follows:
\begin{itemize}
\item 
$R(k)=\Ga(R(k-1), i(R(k-1)))$
and $i_{k-1}=i(R(k-1))$,
in particular,
$R(k)$ satisfies the hypotheses of Fact~\ref{l.retangulo}, 
\item
$R^{k}\subset R^{k-1}\subset \cdots \subset R^1\subset R(0)=R_n(x)$
and $R^k=f_t^{-i_0-\cdots -i_{k-1}}(R(k))$.
\end{itemize}
We define
$i_k=i(R(k))$,
$R(k+1)=\Ga(R(k), i_k)$ and
$R^{k+1}=f_t^{-i_0-\cdots -i_{k}}(R(k+1))$,
completing the inductive process.
\end{demo}















==> seqs.tex <==

\subsection{Proof of Theorem~\ref{t.HssubsetHp}:
the inclusion $H^+(S,f_{t})\subset H(P, f_t)$}
\label{ss.newingredients}


Consider the homoclinic point $x_t=(-1/2,t,0)$ of $P$ for $f_t$
and the fundamental domains
$\De^+_t(i) =
\Phi^{-i} (\De^+_t(0))$, $i\ge 0$,
where
$\De_t^+(0)=
[\Phi^{-1}(t), t]$.
Let
$\ka_t$
be the first $k \in \NN$ such that 
$\Phi^{k}(\De_t^+(0))\subset [1-t,1]$. 
Observing that, for small $t>0$, 
$|\Phi^{k_t}(\De_t^{-})|\le t\, (1-\la)$ and
$|\De_t^+|\le (t^2)/\la$, we get, 
using the Bounded Distortion Lemma~\ref{f.distorcao},
\begin{equation}
\label{f.kappa_t}
  (\Phi^{\ka_t})^\prime(x) <  \frac{1-\la}{\la \, t}\, e^{K},
\quad
\mbox{for all $x\in \De_t^+(0)$.}
\end{equation}
Denote by $\de_t^i$ the length of
$\De^+_t(i)$.
Since the derivative of $\Phi$ near $0$ is close to $1$
and strictly bigger than $1$ in $(0,t]$,
for small $t$, we have that
\begin{equation}
\label{f.9/10}
\displaystyle{\de_t^0 \geq \de_t^i \geq \frac{9\,\de_t^0}{10}},
\quad
i = 1,\dots,4.
\quad
\mbox{In particular,}
\quad
 \sum_{i = 0}^4 \de_t^i \in [4 \de_t^0, 5 \de_t^0].
\end{equation}

We now construct a family 
$\cH_t$
of homoclinic points of
$P$ for $f_t$ such that
the set $\{ y\colon \, (x,y,z)\in \cH_t\}$  
is dense in $\De_t^+(0)$:


\begin{prop}
\label{p.sexsdensas}
For every small
$t>0$ there are sequences of homoclinic points of 
$P$ of the form 
$(b_{i_1,i_2,\dots, i_m,k},x_{i_1,i_2,\dots, i_m,k}, 0)_{k\in \NN^*}$,
$b_{i_1,i_2,\dots, i_m,k} \in [-1,0]$,
such that
\begin{description}
\item{{\bf (H1)}}
$x_{i_1,i_2,\dots, i_m,k}\in \bigcup_{i=0}^4 \De_t^+(i) = \De_t$,
\item{{\bf (H2)}}
$x_{i_1,i_2,\dots, i_m,k}\to 
x_{i_1,i_2,\dots, i_m}$ 
as $k\to \infty$,
\item{{\bf (H3)}}
$x_{i_1,i_2,\dots, i_m,0} <x_{i_1,i_2,\dots, (i_m-1)}$
for every $i_m\ge 1$,
\item{{\bf (H4)}} 
$\mbox{{\rm diam}}(x_{i_1,i_2,\dots, i_m,k})\to 0$ as $m\to \infty$,
\item{{\bf (H5)}}
$(x_i)$ is increasing and $x_i\to t^-$ as $i\to \infty$,
\item{{\bf (H6)}}
$x_0\in \De_t^+(1)$ and  $x_0 \not\in \De_t^+(0)$.
\end{description}
\end{prop}

This proposition will be proved in Section~\ref{sss.sexsdensas}.
From the proposition one gets the following:

\begin{coro}
\label{c.chato}
The set
$\cH_t = \bigcup_{n,k \in \NN^*}(x_{i_1,i_2,\dots, i_k,n})$ 
contains a  dense subset of $\De^+_t(0)$.
\end{coro}


\begin{demo}
The proof of is identical to \cite[Lemma???????]{Dnon},
FALTA REFERENCIA!
 but we repeat it here for
completeness.
Take any point $x\in \De_t^+(0)$. 
If
$x \in \cH_t$ there is nothing to prove.
Otherwise, 
by (H5) and (H6), there is 
$i_1 > 1$ with
$x_{(i_1-1)} < x < x_{i_1}.$ 
Analogously, 
by (H2) and (H3),  
there is $i_2>1$ with 
$x_{i_1,(i_2-1)} < x < x_{i_1,i_2}.$
Inductively,  using (H2) and (H3) as above,
we get a sequence $\{i_k\}$, $i_k > 1$,
such that, for all $k$, 
$
x_{i_1,\dots,(i_k-1)} < x < x_{i_1,\dots,i_k}.
$
Finally, from (H4), 
$\lim_{k \to \infty} x_{i_1,\dots,i_k} = x$, ending the proof of the
lemma.
\end{demo}





\subsubsection{Proof of Theorem~\ref{t.HssubsetHp}}
The deduction of Theorem~\ref{t.HssubsetHp} from
Corollary~\ref{c.chato} follows as in \cite{Dnon}.
For completeness, we sketch here this proof.
%\begin{figure}[hbtp]
%\centering
%
%\psfrag{Bt}{$B_t$}
%\psfrag{Q}{$0 = Q$}
%\psfrag{P}{$0 = P$}
%\psfrag{t}{$t$}
%\psfrag{-t}{$-t$}
%\psfrag{1}{$H^{-1}(t)$}
%\psfrag{2}{$H^{-2}(t)$}
%\psfrag{3}{$H^{-3}(t)$}
%\psfrag{4}{$H^{-4}(t)$}
%\psfrag{a}{$(x_i)_i$}
%\psfrag{a1}{$(y_i)_i$}
%\psfrag{b}{$(x_{2,i})_i$}
%\psfrag{b1}{$(y_{3,i})_i$}
%\psfrag{c}{$(x_{1,i})_i$}
%\psfrag{d}{$(x_{1,2,i})_i$}
%\psfrag{d1}{$(y_{1,2,i})_i$}
%\psfrag{x3}{$x_3$}
%\psfrag{x31}{$x_{3,1}$}
%\psfrag{x31i}{$(x_{3,1,i})_i$}
%\psfrag{x311i}{$(x_{3,1,1,i})_i$}
%\psfrag{x312i}{$(x_{3,1,2,i})_i$}
%\includegraphics[height=3in]{sexs.eps}
%\caption{Esquema de $(x_{i_1,i_2,\dots, i_m,k})_k$ e $(y_{i_1,i_2,\dots, i_m,k})_k$}
%\label{seqs}
%\end{figure}
Consider any $w \in W^u(S,f_t)\pfrk W^{ss}(S,f_t)$.
By replacing $w$ by some iterate of it, we can assume that
$w=(x,0,0)$,  $|x| small$.
We prove that, for  every $\ve>0$, 
the square
$S(\ve)=[x-\ve,x+\ve] \times (0,\ve)\times \{0\}$ 
contained in $W^s(P,f_t)$ transversely intersects 
$W^u(P,f_t)$.
This immediately implies
that $w\in H(P,f_t)$.
The configuration of the cycle and the $\la$-lemma
imply that there is $n(\ve)>0$ such that
$f_t^{-n(\ve)}(S(\ve)$
contains a disk 
$S^\prime(\ve)$
of the form
$$
S^\prime(\ve)= [-1,1]
\times (\bar y -\xi, \bar y +\xi)
\times \{\bar z\},
$$
for some small $\xi>0$ and $\bar y\in (1-t,1)$.
Let $m\in \NN$ be such that
$\Phi^{-m}(\bar y)\in \De_t^+(0)$.
Thus $f_t^{-m}(S^\prime(\ve))$
contains the strip 
$$
\hat S(\ve)=
[-1,1] \times 
(\Phi^{-m}(\bar y-\xi), 
\Phi^{-m}(\bar y+\xi)
\times\{\la_u^{-m}\, \bar z\}
\subset
W^s(P,f_t).
$$
Since $\Phi^{-m}(\bar y)$ belongs to $\De_t^+(0)$,
Corollary~\ref{c.chato} implies that
$\hat S(\ve)$ meets $W^u(P,f_t)$. Thus $\hat S(\ve)$ contains 
a homoclinic point of $P$ and the same holds for $S(\ve)$.
\hfill
$\Box$

\subsubsection{Proof of 
Proposition~\ref{p.sexsdensas}: Sequences of homoclinic points:}
\label{sss.sexsdensas}

Consider the interval 
 $[1-\eta_t, 1]$, where
$\eta_t=\de_t^1+\de_t^0.$
Define $\alpha_t$ as the first natural number $\alpha$  with
$$
\Phi^{\ka_t+\alpha}(\De_t^+(0))\subset [1-\eta_t, 1].
$$
Observe that $|\De_t^+(0)| = \de_t^0<t^2$ 
and $\de_t^1<\de_t^0$. Thus 
$\eta_t <  2\,\de_t^0< 2\, t^2<\la\, t$.
Since
$\Phi^{\ka_t}(\Phi^{-1}(t))\in [1-t, 1-\la\, t]$ and
$(1-\la\,t)<(1-\eta_t)$,
we get that $\alpha_t\ge 1$ for every small
$t$.
Observe also that
$t^2 <\eta_t<2 \,t^2$,
where the first inequality follows from (\ref{f.9/10})
and
$\de_t^0>3t^2/4$ if $t$ is small enough.

\begin{lemm}
\label{l.lambdaalphat}
For every small $t>0$
$\la^{\alpha_t}\le  (2\, t)/\la.$
\end{lemm}

\begin{demo}
By definition of $\ka_t$ and $\alpha_t$, $\Phi^{\ka_t}(\De_t^+(0))=
[1-e_t^-,1-e_t^+]$, where
$e_t^-\in [\la\, t, t]$, and
$\Phi^{\alpha_t}(1-e_t^-)\in [1-\eta_t, 1-\la\, \eta_t].$
Thus,
since
$\Phi$ is affine near $1$,
$\la^{\alpha_t}(e_t^-) \in (0,\eta_t].$
Thus, from $t^2<\eta_t<2\,t^2$ and 
$\la\, t \le e_t^-\le t$,
$$
\la^{\alpha_t} \leq \frac{\eta_t}{e_t^-} \leq 
\frac{2\, t}{\la},
$$
ending the proof of the lemma.
\end{demo}

Next contraction lemma is necessary for getting 
(H4) in  Proposition~\ref{p.sexsdensas} and 
along the inductive definition of the sequences
$(x_{i_1,i_2,\dots, i_m,k})_k$.

\begin{lemm}
\label{l.derivada<1/2}
$L = \max \{ (\Phi^{\ka_t+\alpha_t+j})^\prime (x);\,
x\in \cup_{i=0}^4 \De^+_t(i) \mbox{ and } j\ge 0\}< \frac{1}{2}.$
\end{lemm}

\begin{demo}
Since $\Phi$ is a contraction near $1$,
it is enough to compute the estimate when $j=0$.
We split the trajectory of a point $x\in  \De^+_t(i)$
going from $\De_t^+(i)$ to $[1-\eta_t,1)$ as follows:
{\bf (i)}
$i$ iterates,
$i\le 4$, for $x$  going  from $\De^+_t(i)$ to
$D^+_t(0);$
{\bf (ii)}
$\ka_t$ iterates for $\Phi^i(x)$ 
going from $\De^+_t(0)$ to
$\De^-_t$; and 
{\bf (iii)}
$\alpha_t$ iterates  for  $\Phi^{\ka_t+i}(x)$ 
going from $\De^-_t$ to
$ [1-\eta_t,1].$ 
This  construction involves
$(i + \ka_t + \alpha_t)$ iterations of $x$ by $\Phi$, that is,
we need to remove the last $i$  
iterations, 
corresponding to a contraction by $\la^i$.
We claim that
\begin{equation}
L
\leq 
\underbrace{((2\,t+1)^4)}_{(\mbox{{\bf a}})} 
\, 
\underbrace{
\frac{e^{K}\,(1 - \la)}{\la \, t} 
\,
\la^{\alpha_t}
}_{(\mbox{{\bf b}})}
 \,
\underbrace{\frac{1}{\la^4}}_{(\mbox{{\bf c}})},
\end{equation}
corresponding
(\mbox{{\bf a}}) to the expansion of the first
$i$ iterates by $\Phi$
(just observe that in $[0,t]$ the derivative of 
$\Phi$ is upper bounded by
$(2\,t+1)$  and that $i\le 4$),
(\mbox{{\bf b}})
to an upper bound of the derivative of
$\Phi^{\ka_t+\alpha_t}$, 
recall (\ref{f.kappa_t}), and
(\mbox{{\bf c}})  to the  $i$ ($i \leq 4$)
negative  iterates of $\Phi$ close to $1$.
By (SN), Lemma \ref{l.lambdaalphat}, and the fact that 
 ${(2\,t+1)}^4 < 2$ if $t>0$ is small, we get
$$
%\begin{equation}
L
\leq
 ({(2\,t+1)}^4) \, 
\frac{e^{K}\,(1 - \la)}{\la\, t} \,
\frac{2\, t}{\la} \, \frac{1}{\la^4} 
= {(2\,t+1)}^4 \, \frac{2\,(1 - \la)\, e^{K}}{\la^6}
\leq 4\, e^{K}\,\frac{(1 - \la)}{\la^6} < \frac{1}{2},
%\end{equation}
$$
\end{demo}


\paragraph{Construction of the sequences 
$(x_{i_1,i_2,\dots, i_m, k})$.} 
To construct  the 
sequences $(x_{i_1,i_2,\dots, i_m, k}),$
we need the following algorithm 
about the creation of homoclinic points,
which is a consequence of the definition of
the unfolding of the heterodimensional cycle.



\begin{algo}
\label{a.algo2}
Let $(x,y,0)$, $y\in [0,t]$, be a homoclinic point of
$P$ (for $f_t$) such that
$\{(x,y)\}\times [-1,1]\subset W^u(P,f_t)$.
Then, for every $m$ with
$\Phi^m(y)\in (1-t,1)$,
 there is a homoclinic point
of $P$ of the form
$(\bar x, \Phi^m(y)+t-1,0)$
such that
$\{(\bar x, \Phi^m(y)+t-1)\}\times [-1,1]\subset
W^u(P,f_t)$.
\end{algo}
 

Consider the homoclinic point
$(-1/2,t,0)$ of $P$ for $f_t$
(satisfying Algorithm~\ref{a.algo2}) and
the sequences
$(y_i)_{i \in \NN^*}$ and 
$(x_i)_{i \in \NN^*}$ defined by
$$
y_i= \Phi^{\ka_t+ \alpha_t + i}(t) \quad 
\mbox{and}
\quad
x_i=(t-1)+y_i,
\quad
y_i\to 1
\quad
\mbox{and}
\quad
x_i \to t.
$$
Observe that, for each $i\ge 0$, there is a homoclinic
point $(b_i,x_i,0)$ of $P$ verifying Algorithm~\ref{a.algo2}.
Also,
by the definitions of
$\alpha_t$ and $\ka_t$, 
$y_i\in [1-\eta_t,1]$ for all $i\ge 0$.
Thus, since $\eta_t=\de_t^0+\de_t^1$, one has
\begin{equation}
\label{f.x_iinDt}
x_i\in [t- \eta_t,t] = [t-(\de_t^1+\de_t^0),t]
 = \De_t^+(1)\cup \De_t^+(0).
\end{equation}



\begin{lemm}
\label{l.h6} 
The sequence
$(x_i)_{i \in \NN^*}$ verifies (H5) and (H6).
\end{lemm}

\begin{demo}
%By (\ref{f.x_iinDt}),
%it is enough to see that 
%$x_0\not \in \De_t^+(0)$. 
Condition (H5) follows by definition. 
To prove (H6), $x_0 =  y_0 +(1-t) \in (\De_t^+(1)\setminus \De_t^+(0))$,
observe that,
by  construction, 
$x_0\in [t-\eta_t, t- \la \, \eta_t]$
and
$\De_t^+(1)= [t-\eta_t, t-\de_t^0]$. Thus, we need
to check that
$\la\, \eta_t
=\la\,(\de_t^0+\de_t^1)>\de_t^0$.
This inequality folllows from $\de_t^0 >\de_t^1$, (\ref{f.9/10}) and (SN), 
observing that
$$
\frac{\de_t^0}{\de_t^0+\de_t^1}< \frac{\de_t^0}{2\, \de_t^1}<
\frac{\de_t^0}{2\, (9/10) \, \de_t^0}=\frac{10}{18}<
\frac{2}{3}
<\la.
$$
The proof of the lemma is now complete.
\end{demo}

We now proceed with the construction  of
the sequences in Proposition~\ref{p.sexsdensas}.
For each
$j\in \NN^*$, 
define the sequences
$(y_{j,i})_{i \in \NN^*}$ and 
$(x_{j,i})_{i \in \NN^*}$ as follows,
$$
y_{j,i}=\Phi^{\ka_t+\alpha_t+j}(x_i)
\quad
\mbox{and}
\quad
x_{j,i}=(t-1) + y_{j,i}.
$$
We claim that
$y_{j,i} \to y_j$ and, consequently,
$x_{j,i} \to x_j$, as $i \to \infty$. For that just observe that
$\lim_{i\to\infty}x_i=t$, thus, by
continuity,
$
\lim_{i\to\infty}y_{j,i} = 
\lim_{i\to\infty}\Phi^{\ka_t+\alpha_t+j}(x_i)=
\Phi^{\ka_t+\alpha_t+j}(t)=y_{j}.$

\begin{lemm}
The points $(x_{j,i})_i$ belong to
$\cup_{i=0}^4 \De_t^+(i)$
for all  $i, j\in\NN \cup \{0\}$. 
\label{l.step2}
\end{lemm}

\begin{demo}
By construction, the sequences $(x_{j,i})_i$ are increasing, thus
it is enough to prove that $x_{0,0}\in  \cup_{i=0}^4 \De_t^+(i)$.
Let $d_0=(t-x_0)$ be the diameter of $(x_i)_{i\in \NN^*}$.
By (\ref{f.x_iinDt}),
 $d_0<\de_t^0+\de_t^1$.
Let 
$d_1=|x_0-x_{0,0}|$
be the diameter of 
the sequence $(x_{0,i}=\Phi^{\ka_t+\alpha_t}(x_i)+(t-1))_i$, 
which is equal to the diameter of $(\Phi^{\ka_t+\alpha_t}(x_i))_i$.
Therefore,
since $(x_i)_i\subset \De_t^+(0)\cup \De_t^+(1)$,
by Lemma~\ref{l.derivada<1/2},
the diameter
$d_1$  is bounded by
\begin{equation}  
\label{e.step2}
d_1\le L \, d_0<   L\,(\delta^0_t+\delta^1_t)/2< 
(2\, \delta^0_t)/2<
\delta^0_t.
\end{equation}
Since $x_0\in \De_t^+(1)$ (see Lemma~\ref{l.h6}),
in order to prove  $x_{0,0}\in  \cup_{i=0}^4 \De_t^+(i),$
it is enough to see that
$$
x_{0,0}
=x_0-d_1>
x_0-(\de_t^2+\de_t^3+\de_t^4)
\Longleftrightarrow
d_1<(\de_t^2+\de_t^3+\de_t^4),
$$
which immediately follows from
$\de_t^2+\de_t^3+\de_t^4> \de_t^0>d_1$, the first inequality being consequence
of
$\de_t^i>(9\, \de_t^0)/(10)$, see (\ref{f.9/10}), and the last from 
(\ref{e.step2}).
This ends the proof of the lemma.  
\end{demo}

Suppose now inductively defined 
sequences
 $(y_{i_i,i_2,\dots,i_m,i})_{i\in \NN^*}$ and 
$(x_{i_i,i_2,\dots,i_m,i})_{i\in\NN^*}$
by
$$
y_{i_1,i_2,\dots,i_m,i}=\Phi^{\ka_t+\alpha_t+i_1}
(x_{i_2,\dots,i_m,i})
\quad
\mbox{and}
\quad
x_{i_1,i_2,\dots,i_m,i}=
(t-1) + y_{i_1,i_2,\dots,i_m,i},
$$
satisfying conditions
(H1), (H2), (H3) and
\begin{description}
\item
{{\bf (H2b)}}
$(y_{i_1,i_2,\dots,i_m,i})_i \to y_{i_i,i_2,\dots,i_m}$
as $i\to \infty$,
\item
{{\bf (H3b)}}
$y_{i_1,i_2,\dots,i_m,0}<  y_{i_i,i_2,\dots,(i_m-1)}$
for all  $i_m\ge 1$.
\item{{\bf (H4b)}}
Let  $d_m$, $m\ge 0$, be the  diameter of the  sequence 
$(x_{\underbrace{0,\dots,0,i}_{m \, 0's}})_{i}$. 
Then  $d_m\le  (d_{m-1})/2$.
\end{description}

Observe that
(H2) and (H2b) (resp. (H3) and (H3b)) are equivalent.
Notice that, for $m=1$,
(H1) follows from Lemma~\ref{l.step2}, (H2) and (H2b) from definition, 
and (H4b) from (\ref{e.step2}).
To check (H3b), $y_{i,0}<y_{i-1}$, 
recall that,
by Lemma~\ref{l.h6},
$x_0<\Phi^{-1}(t)<t$, thus
$$
y_{i-1}=\Phi^{\ka_t+\alpha_t+i-1}(t)=
\Phi^{\ka_t+\alpha_t+i}(\Phi^{-1}(t))>
\Phi^{\ka_t+\alpha_t+i}(x_0)=y_{i,0}.
$$

To simplify the notation we say that
the sequence 
$(x_{i_i,i_2,\dots,i_m,i})_{i\in\NN^*}$
is of generation $m$.

\begin{lemm}
\label{l.i4h4}
Property (H4b) implies (H4) 
in  Proposition~\ref{p.sexsdensas}.
\end{lemm}

\begin{demo}
Observe that, by construction,
the diameters of the  sequence of generation $m$ are
bounded by the diameter $d_m$ of
$(x_{0,\dots,0,i})_{i\in\NN^*}$.  Thus, inductively, 
$d_m\le (1/2) \, d_{m-1}\le (1/2)^{m} \, d_0.$
\end{demo}

Keeping in mind Lemma~\ref{l.h6}, in order to
to prove Proposition~\ref{p.sexsdensas} it suffices to
see that the sequences above verify (H1), (H2b), (H3b) and (H4b). 
We argue inductively
on the generation of the sequences and assume satisfied these conditions
for sequences of generation less than or equal to
$m$.

To verify 
(H2b) 
for the sequences of generation $m+1$.
note that, by induction,
$(y_{i_1,i_2,\dots,i_m,i})_i \to y_{i_1,i_2,\dots,i_m}$. Thus,
by continuity of $\Phi$ and by definition,
$$
(y_{j,i_1,i_2,\dots,i_m,i}))_i=
(\Phi^{\ka_t+\alpha_t+j}(x_{i_1,i_2,\dots,i_m,i}))_i 
\to 
\Phi^{\ka_t+\alpha_t+j}(x_{i_1,i_2,\dots,i_m})
=y_{j,i_1,i_2,\dots,i_m}.
$$
To prove   (H3b) observe that, by induction,
$
x_{i_1,i_2,\dots,i_m,0}
<x_{i_1,i_2,\dots,i_m-1}.
$
Thus,  since $\Phi$ is increasing,
$$
y_{j,i_1,i_2,\dots,i_m,0}=
\Phi^{\ka_t+\alpha_t+j}(x_{i_1,i_2,\dots,i_m,0})
<
\Phi^{\ka_t+\alpha_t+j}
(x_{i_1,i_2,\dots,i_m-1})=
y_{j,i_1,i_2,\dots,i_m-1}.
$$
Finally, to prove (H4b) recall that
$(y_{0,\dots,0,i})_i=(\Phi^{\ka_t+\alpha_t}
(x_{0,\dots,0,i}))_i.$
Since, by the induction hypotheses (H1), 
$x_{0,\dots,0,i}\in  \cup_{i=0}^4 \De_t^+(i)$, 
Lemma~\ref{l.derivada<1/2} 
and the fact that the sequences 
$(y_{0,\dots,0,i})$ and  
$(x_{0,\dots,0,i})$ have the same diameter
imply that
$$
d_{m+1} =\mbox{diam}(\underbrace{
                                 (y_{0,\dots,0,i})_i}_{(m+1)\, 0's})
=
\mbox{diam}((\Phi^{\ka_t+\alpha_t}
                    (\underbrace{(x_{0,\dots,0,i})_i)}_{m \, 0's})
=L \,
\mbox{diam}
((x_{0,\dots,0,i}))_i) = L \, d_m \le \frac{d_m}{2},
$$
which ends the proof of (H4b).
Condition (H1) for sequences of generation $(m+1)$ follows from:

\begin{lemm}
Suppose that the sequences 
of generation $m$ verify 
(H4b) and (H1). Then the sequences of generation $(m+1)$ verify
(H1).
\end{lemm}

\begin{demo}
It is enough to see that, for every $m$,
$
\sum_{i=0}^m d_m < 4 \de_t^0 < \sum_{i=0}^{4} \de_t^i,
$
where the last inequality follows from (\ref{f.9/10}).
By induction and
Lemma~\ref{l.h6},
we have
$$
\sum_{i=0}^m d_m \le
\sum_{i=0}^{m-1} (1/2)^i \, d_0 \le 
\sum_{i=0}^{m-1} (1/2)^i \, 
 (\de_t^0+\de_t^1) \le 
\frac{1}{1-2}\, (\de_t^0+\de_t^1)<
{2}(\de_t^0+\de_t^1)< 4\de_t^0,
$$
ending the proof of the lemma.
\end{demo}

The construction of the sequences  
$(x_{i_i,i_2,\dots,i_m,i})_{i\in\NN^*}$ of 
Proposition~\ref{p.sexsdensas} is now complete.













==> snhc.tex <==

\section{Saddle-node heterodimensional cycles}
\label{s.selano}

In this section, we consider 
{\em saddle-node heterodimensional cycles.\/}
For that, in the definition of the heterodimensional cycle in 
Section~\ref{s.heterodimensional}, we replace the function $F$ (defining the
central dynamics) by a one parameter family of 
maps 
$\Phi_s\colon [-1,2]\to (-1,2)$ such that: 
\begin{itemize}
\item
For every $s$, 
the point $1$ is an attracting hyperbolic point of $\Phi_s$ 
and $\Phi_s$ is linearizable in a neighborhood
of $1$ (independent of $s$). We denote by $0<\la<1$ the eigenvalue
of $\Phi_s$ at $1$.
\item
Locally in $0$, the map $\Phi_s$ is of the form
$\Phi_s(x)= x+x^2 -s$.
Thus, for $s>0$, $\Phi_s$ has
two hyperbolic fixed points
$\pm \sqrt{s}$ (an attractor and a repellor)
collapsing at $s=0$. Moreover,  $s<0$,
$\Phi_s$ has no fixed points close to $0$. 
\item
Every $\Phi_s$ is strictly increasing and
has no fixed points different from
$1$ and $\pm\sqrt{s}$.
\end{itemize}

%\subsection{Two parameter families of diffeomorphisms}
%\label{ss.twoparameter}

We now define, as in Section~\ref{s.heterodimensional}, a two parameter
family of diffeomorphisms
$f_{t,s}$: 
the parameters $t$ and $s$ describing 
the motion of the unstable manifold
of $P$ and the unfolding of the
saddle-node  (i.e., $f_{t,s}(0,y,0)=(0, \Phi_s(y),0)$), 
respectively.
Observe that 
$P=(0,1,0)$, $S^-_s=(0,-\sqrt{s},0)$ and $S^+_s=(0,\sqrt{s},0)$
($s\ge 0$)
are fixed points of
$f_{t,s}$.



We let $f_t=f_{t,0}$.
For the saddle-node  $S=(0,0,0)$ of $f_t$ there are
defined the stable and unstable manifolds 
(denoted $W^s(S,f_t)$ and $W^u(S,f_t)$)
and the strong stable and unstable manifolds
(denoted by $W^{ss}(S,f_t)$ and
$W^{uu}(S,f_t)$).
Observe that
$W^s(S,f_t)$ and $W^u(S,f_t)$
are
two-manifolds with boundary and 
$W^{ss}(S,f_t)$ and
$W^{uu}(S,f_t)$ have 
both dimension one. 
Notice that
$$
\begin{array}{ll}
&\{0\}\times [0,1)\times [-1,1]
\subset W^u(S,f_t),
\quad
[-1,1]\times [-2,0]\times \{0\}
\subset W^s(S,f_t),
\\
&[-1,1]\times \{(0,0)\}
\subset W^{ss}(S,f_t),
\quad
\{(0,0)\} \times [-1,1]
\subset W^{uu}(S,f_t).
\end{array}
$$
Keeping in mind these relations, we have that, 
\begin{itemize}
\item
for all $t$,
$W^u(S,f_t)$
meets transversely  $W^s(P,f_t)$ 
throughout the segment $\{0\}\times (0,1)\times \{0\}$.
\item
for $t=0$,
$W^u(P,f_0)$ meets quasi-transversely  $W^{ss}(S,f_0)$
along the orbit of
$(-1/2,0,0)$, 
\item
The point $(-1/2,t,0)$ is a transverse homoclinic point of $P$ for
$f_t$ and 
$(-1/2,0,0)$ is a point of transverse intersection
between $W^{ss}(S,f_t)$ and $W^u(S,f_t)$.
\end{itemize}
In this case, we say that
the arc 
$f_{t}=f_{t,0}$
has a {\em heterodimensional saddle-node cycle\/}
associated to $P$ and 
$S$ at $t=0$.
This cycle can be thought as a 
a limit case of the heterodimensional
cycles in Section~\ref{s.heterodimensional} where the derivative of the point
of index two $Q$ is $1^+$.

The two-fold behavior of the saddle-node $S$, as
a point of index two and one simultaneously, 
leads us to consider, for small positive $t$, 
the {\em lateral homoclinic classes of $S$\/} defined by 
$$
H^+(S,f_t)=\overline{W^u(S,f_t) \pfrk
W^{ss}(S,f_t)}
\quad
\mbox{and}
\quad 
H^-(S,f_t)=\overline{W^s(S,f_t) \pfrk
W^{uu}(S,f_t)}.
$$
As in the case of the usual homoclinic classes, we have that:

\begin{prop}
\label{p.lateral}
For every small $t>0$,
$H^+(S,f_t)$ (resp. 
$H^-(S,f_t)$)
is transitive and the periodic points of index
two (resp. one) form a dense subset of it. 
\end{prop}

Consider a neighborhood $W$ of the saddle-node heterodimensional cycle
defined 
as in Section~\ref{s.pontosnaoerrantes} and denote by $\Ups_t$
 the maximal
invariant set of $f_t$ in $W$.

\begin{theor}
\label{t.latlat}
For every small $t>0$, one has that
$H(P,f_t)\subset H^+(S,f_t)$ and $\Ups_t\subset H(S^+,f_t)$.
\end{theor}

The proof of Theorem~\ref{t.latlat}
follows as the one of
Theorem~\ref{t.lat}, the only difficulty being to
redefine appropriately the one-dimensional dynamics
associated to the cycle
(recall Section~\ref{s.dinamica1dim}). 
This will be 
briefly done in the next section.

To get the inclusion
$H^+(S,f_t)\subset H(P,f_t)$
we need  the following distortion
assumption for the saddle-node map $\Phi=\Phi_0$:

\begin{description} 
\item
{\bf (SN)}
$
\displaystyle{   
\frac{4 \, e^{K}\, (1-\la)}{\la^6}  < \frac{1}{2}}$,
where
$\la\in (2/3,1)$.
\end{description}

\begin{theor}
\label{t.HssubsetHp}
The inclusion 
$H^+(S,f_{t})\subset H(P, f_t)$ holds for all small positive 
$t>0$ 
\end{theor}
To prove this theorem we need new ingredients that will be  introduced in
Section~\ref{ss.newingredients}.



\subsection{One-dimensional dynamics for the  saddle-node cycle}
\label{ss.1dim}
We now
adapt the definitions of  scaled fundamental domains,
transitions and returns for the saddle-node heterodimensional cycles.
%We assume that $G$ verifies the following conditions
%(playing the role of conditions 
%(F1--F3) in Section~\ref{s.dinamica1dim})
%\begin{description}
%\item{{\bf (G1)}}
%$\displaystyle{
%\frac{8 \,  e^{-K}\, (1-\la)}{\la^4} \, < \,\frac{1}{2},
%}$
%where $K>0$ is an upper bound of 
%$\displaystyle{\frac{G''(x)}{G'(x)}}$,
%\item{{\bf (G2)}}
%$\displaystyle{\la>\frac{2}{3}}.$
%\end{description}
Let $\Phi=\Phi_0$.
As in Section~\ref{s.dinamica1dim}, for each $t>0$,  
define the
fundamental domains $D_t^-=[1-t, 1-\la\, t]$ 
and $D_t^+=[a_t,b_t]$, where $D_t^+$ is the first backward iterate of
$D_t^-$ by $\Phi$ contained in $[0,t]$.
We have 
$\Phi^{k_t}(D_t^+)=D_t^-$, for some $k_t\in \NN$.
Observe that $|D_t^-| = t\, (1 - \la)$ and,
since $b_t\in (0,t]$,
$|D_t^+| \le t^2$.
For small $t>0$,
define the {\em transition\/}
$\mfT_t$ and the map $\mfG_t$ by
$$
\mfT_t \colon  D_t^+ \rightarrow D_t^-,\,\,\,
x\mapsto \mfT_t(x)=\Phi^{k_t}(x)\quad
\mbox{and}
\quad
\mfG_t \colon D_t^+ \to [0, t(1-\lambda)],
\,\,\,
x\mapsto \mfG_t(x)=\mfT_t(x)+t.
$$



\begin{lemm}
\label{l.mfTtexpansora}
The maps $\mfT_t$ and 
$\mfG_t$ are uniformly expanding for all small $t>0$.
\end{lemm}

\begin{demo}
It suffices to see that
$(\Phi^{k_t})^\prime(z)>1$ for all $z\in D_t^+$.
We use the following  standard
lemma:

\begin{bdl}
\label{f.distorcao}
Let 
$K>0$ be an upper bound of 
$|\Phi''(x)|/|\Phi'(x)|$,
$x\in [-1,2]$.
Then,
for every pair of points 
$z, y\in D_t^+$  and every small $t>0$, it holds 
$$
e^{-K}
\le
\frac{(\Phi^{k_t})^\prime(z)}
{(\Phi^{k_t})^\prime(y)}
\le 
e^{K}.
$$
\end{bdl}
The lemma now follows by the mean value theorem, taking 
$y$ with
$(\Phi^{k_t})^\prime(y)=|D^-t|/|D_t^+|\ge (1-\la)/t$.
Thus, if $t$ is small,
$(\Phi^{k_t})^\prime(z)\ge 
(e^{-K}\,(1-\la))/t>1$, for all $z\in D_t^+$. 
\end{demo}


As in
Section~\ref{s.dinamica1dim},
given 
$x\in (a_t, b_t]=\tilde D_t^+$, 
let
$i(x) \in \ZZ$ be the first
$i$ with
$\Phi^i(\mfG_t(x)) \in D^+_t.$


\begin{lemm} 
\label{l.left}
There exists $i_0>0$ such that
$i(x)\ge i_0$ for all $x\in \tilde{D}_t^+$.
\end{lemm}

\begin{demo}
To prove the lemma it is enough to see that
$\mfG_t(D_t^+)\subset (0,a_t)$.
By definition,
$\mfG_t(D_t^+) = [0,(1 - \lambda)\, t]$.
Observe that, if $t$ is small enough,
$$
\Phi^2((1-\la) \, t)= 
\Phi((1-\la)\,t +(1-\la)^2\,t^2) = 
(1-\la)\,t +(1-\la)^2\,t^2 + \mbox{h.o.t}
< t.
$$
Thus,
the right extreme of $\Phi^2((1 - \lambda) t)$ of 
$\Phi^2(\mfG_t(D_t^+))$ 
is less than
$t$. In particular, the right extreme of $\mfG_t(D_t^+)$
is less than 
$\Phi^{-2}(t)$, and the 
the lemma follows  from $D_t^+ \subset (\Phi^{-2}(t),t]$.
\end{demo}

The {\em  return map\/} $\mfR_t$  is now defined by
$$
\mfR_t\colon \tilde D^+_t \rightarrow D^+_t,
\quad
\mfR_t(x)=\Phi^{i(x)}(\mfG_t)(x)=\Phi^{i(x)}(\mfT_t(x)+t).
$$ 
As in the case of the map $R_t$ in 
Section~\ref{s.dinamica1dim}, 
for each $i\ge i_0$, there is
$\de_i\in \tilde{D}_t^+$ with  $\mfG_t(\de_{i}) = \Phi^{-i}(a_t)$.
In this way, we get 
a decreasing sequence $(\de_i)_{i\ge i_0}$ with $\de_i\to a_t$,
and intervals
$J_i=[\de_{i+1}, \de_i]$, $i > i_0$, and
$J_{i_0} = [\de_{i_0},b_t]$ such that
$\mfR_t$ is continuous and 
increasing in the interior of each $J_i$.
Extending $\mfR_t$ continuously to the whole $J_i$ we
get a bi-valuated map with
$\mfR_t(\de_i)=\{a_t,b_t\}$ for all $i>i_0$.


\begin{lemm}
\label{l.mfRtexpansora}
The restriction of $\mfR_t$ to each interval
$J_i, i > i_0$, is onto and there is $\ell>1$ such that 
$\mfR_t^\prime(x)>\ell>1$ for all $x\in (a_t,b_t]$
(if $x=\de_i$ this means that the lateral derivatives of
$\mfR_t$ at $x$ are  greater than $\ell$).
Moreover, $\mfG_t(\mfR_t(\de_i)) = 0$
for all $i \geq i_0$.
\end{lemm}

\begin{demo}
The lemma follows as Lemma~\ref{l.mfRtexpansora}
observing that $i_0>0$ (Lemma~\ref{l.left}),
$\mfG_t$ is expanding (Lemma~\ref{l.mfTtexpansora}), 
and that the derivative of
$\Phi$ in $(0,t]$ is bigger than one. 
\end{demo}

Arguing as in 
Section~\ref{s.dinamica1dim}, one gets 
the following lemma (corresponding to Lemma~\ref{l.descont}):

\begin{lemm}
\label{l.WuQt}
Given any subinterval $I$ of
$D_t^+$ there are $x \in I$ and $i\geq 0$ with 
$\mfG_t(\mfR_t^i(x))=0$.
\end{lemm}

\subsection{Lateral Homoclinic classes. Proof of 
Theorem~\ref{t.latlat}}
\label{ss.classeshomoclinicasdaselano}

PRECISA DE UMA SECAO SO PARA ISSO???

To prove Theorem~\ref{t.latlat} we proceed as
in Section~\ref{s.pontosnaoerrantes}.
After redefining vertical strips and segments and  using Lemma~\ref{l.WuQt}
one gets that,
for any
small $t>0$ and any
disk $\chi$ with 
$W^s(P,f_t)\pitchfork \chi\ne \emptyset$,
$W^{ss}(S,f_t)\pitchfork \chi\ne \emptyset$
(recall
Proposition~\ref{p.chi}).
The inclusion
$(H(P,f_t)\cup \Ups_t)\subset H^+(S,f_t)$
follows exactly as $(H(P,f_t)\cup \La_t)\subset H(Q,f_t)$
in the case of heterodimensional cycles.






























